Learning-Augmented Weighted Paging

We consider a natural semi-online model for weighted paging, where at any time the algorithm is given predictions, possibly with errors, about the next arrival of each page. The model is inspired by Belady's classic optimal offline algorithm for unweighted paging, and extends the recently studied model for learning-augmented paging (Lykouris and Vassilvitskii, 2018) to the weighted setting. For the case of perfect predictions, we provide an $\ell$-competitive deterministic and an $O(\log \ell)$-competitive randomized algorithm, where $\ell$ is the number of distinct weight classes. Both these bounds are tight, and imply an $O(\log W)$- and $O(\log \log W)$-competitive ratio, respectively, when the page weights lie between $1$ and $W$. Previously, it was not known how to use these predictions in the weighted setting and only bounds of $k$ and $O(\log k)$ were known, where $k$ is the cache size. Our results also generalize to the interleaved paging setting and to the case of imperfect predictions, with the competitive ratios degrading smoothly from $O(\ell)$ and $O(\log \ell)$ to $O(k)$ and $O(\log k)$, respectively, as the prediction error increases. Our results are based on several insights on structural properties of Belady's algorithm and the sequence of page arrival predictions, and novel potential functions that incorporate these predictions. For the case of unweighted paging, the results imply a very simple potential function based proof of the optimality of Belady's algorithm, which may be of independent interest.

==> model.tex <==
\subsection{Formal model and preliminaries}
\label{sec:model}

There is a universe of $n$ distinct pages and a cache of size $k$. Let $W = \{w_1, \ldots, w_{\ell}\} \subset \bbR^+$ denote a set of $\ell$ distinct weights. Each page $p$ has a weight $w_p \in W$. 
In the standard online model, the current decision on which page to evict must be made without the knowledge of the future requests, whereas an offline algorithm knows the entire request sequence is advance.
In the myopic model considered here, 
at any time, the algorithm only knows the relative order of the next request of each page in $\sigma$.
For example, all these possible future sequences $\tuple{1, 2, 3, 4}$, $\tuple{1, 1, 2, 2, 3, 3, 4, 4}$, and $\tuple{1, 2, 3, 4, 4, 3, 2, 1}$,
look identical to the algorithm.
By the optimality of Belady's algorithm, the myopic model is as powerful as the offline model  for unweighted paging.

Suffices to design a fractional algorithm.
Generic way to convert weighted paging to randomized algorithm with $O(1)$ factor loss.

Should be mention that for allocation problems, we can give small requests etc...

Define competitive ratio somewhere.


==> myopic.tex <==












    










